Real-time face swapping as a tool for understanding infant self-recognition

To study the preference of infants for contingency of movements and familiarity of faces during self-recognition task, we built, as an accurate and instantaneous imitator, a real-time face- swapper for videos. We present a non-constraint face-swapper based on 3D visual tracking that achieves real-time performance through parallel computing. Our imitator system is par- ticularly suited for experiments involving children with Autistic Spectrum Disorder who are often strongly disturbed by the constraints of other methods.

==> bibliography.tex <==
\bibliographystyle{plain}

\begin{thebibliography}{99}

\bibitem{sanefuji2} W. Sanefuji, H. Ohgamu, K. Hashiya, "Preference for peers in infancy",
\emph{Infant Behaviour and Development}, 29(4):584-593, Dec. 2006

\bibitem{bahrick2} L.E. Bahrick, J.S. Watson, "Detection of intermodal proprioceptive-visual contingency as a potential basis of self-perception in infancy".
\emph{ Developmental Psychology}, 21:963-973, 1985

\bibitem{keenan}    J. Keenan , 2004, 
\emph{The Face in the Mirror}, Harper Collins Publishers

\bibitem{rochat} P. Rochat, Ch5,
\emph{Others in Mind}, Cambridge, 2009

\bibitem{sparse template matching}    Y. Matsubara, T. Shakunaga, ''Real-time Object Tracking by Sparse Template Matching'', 
\emph{IPSJ SIG Technical Report}, March 2004


\bibitem{3DModel}   Y. Matsumoto, N. Sasao, T. Suenaga, T. Ogasawara, ''3D Model-based 6-DOF Head Tracking by a Single Camera for Human-Robot Interaction'',
\emph{IEEE ICRA}, 2009


\bibitem{visualTracker} O. Mateo Lozano, K. Otsuka, ''Real-time Visual Tracker by Stream Processing'',
\emph{Journal of Signal Processing Systems}, 57(2), Nov. 2009

\bibitem{faceSwapping}    D. Bitouk, N. Kumar, S. Dhillon, S.K. Nayar, ''Face Swapping: Automatically Replacing Faces in Photographs'',
\emph{SIGGRAPH 2008}, 27(3)


\bibitem{faceAlignment} J.  Zhu, L. Van Gool, S. C.H. Hoi, "Unsupervised Face Alignment by nonrigid Mapping",
\emph{ICCV}, 2009

\bibitem{Uddin}  L. Uddin,  J. Kaplan,  I. Szakcs,  E. Zaidel , M. Iacaboni,  "Self face recognition activates a fronto parietal mirror network in the right hemisphere: an event-related fMRI study", 
\emph{NeuroImage}, 25(3), 926-935, 2005

\bibitem{Goa} Z. Goa, K. Giovanello, K. Smith, D. Shen, L. Gilmore,  "Evidence on the emergence of the brain's default network from 2-week-old to 2-year-old healthy pediatric subjects", 
\emph{ Proceedings of the National Academy of Sciences}, 106(19), 6790-6795, 2009


\end{thebibliography}
